Low Mass Thermal Dilepton Production at NLO in a Weakly Coupled Quark-Gluon Plasma

We present a computation, within weakly-coupled thermal QCD, of the production rate of low invariant mass ($M^2 \sim g^2 T^2$) dileptons, at next-to-leading order (NLO) in the coupling (which is $O(g^3 e^2 T^2)$). This involves extending the NLO calculation of the photon rate which we recently presented to the case of small nonzero photon invariant mass. Numerical results are discussed and tabulated forms and code are provided for inclusion in hydrodynamical models. We find that NLO corrections can increase the dilepton rate by up to 30-40% relative to leading order. We find that the electromagnetic response of the plasma for real photons and for small invariant mass but high energy dilepton pairs (e.g., $M^2 < (300\:\mathrm{MeV})^2$ but $p_T > 1 \: \mathrm{GeV}$) are close enough that dilepton pair measurements really can serve as Ersatz photon measurements. We also present a matching a la Ghisoiu and Laine between our results and results at larger invariant masses.

==> README <==
This directory contains several files needed to compute next-to-leading
order dilepton rates at small invariant mass.
The dilepton rate is written as a sum of four terms:
$$
\Pi^<(K) = \mathcal{B} ( \ln(T/m_D) + C_{22} + C_{12} )
$$
The total rate from inelastic "$1\to 2$" type processes is
$C_{12}$.  At large virtuality this is approximated by a free Born term
and a Born correction.

This code computes $C_{12}$, at leading and next-to-leading order.  
The result is of form
$$
C_{12}[k/T,(k^0-k)/(g^2 T)] = C_{LO} + g C_{NLO}
$$
it presents results for $C_{LO}$ and $C_{NLO}$.
It separately computes the free Born term and its next correction, and
subtracts them from $C_{LO}$.

System requirements:
c compiler (typically gcc)
libraries:  <math.h> and <gsl/gsl_sf_bessel.h> are needed.

Files:
NLO.dat    some data files regarding the NLO corrections to the
	   collision operator
photoNLO.c contains main computational tools.
photoNLO.h gives prototype of the one desired function introduced
	   in photoNLO.c
sample_driver.c very simple example main() which uses the above.

You can compile this simple sample main() using, eg,
gcc -lm -lgsl -lgslcblas photoNLO.c sample_driver.c

The file NLO.dat MUST be in the same directory as the executable when
it is run.

Most users will never need to look inside photoNLO.c, they will just
want to adapt sample_driver.c into something else to suit their
purpose (for instance, to build a table for interpolation).

